VideoClick: Video Object Segmentation with a Single Click

Annotating videos with object segmentation masks typically involves a two stage procedure of drawing polygons per object instance for all the frames and then linking them through time. While simple, this is a very tedious, time consuming and expensive process, making the creation of accurate annotations at scale only possible for well-funded labs. What if we were able to segment an object in the full video with only a single click? This will enable video segmentation at scale with a very low budget opening the door to many applications. Towards this goal, in this paper we propose a bottom up approach where given a single click for each object in a video, we obtain the segmentation masks of these objects in the full video. In particular, we construct a correlation volume that assigns each pixel in a target frame to either one of the objects in the reference frame or the background. We then refine this correlation volume via a recurrent attention module and decode the final segmentation. To evaluate the performance, we label the popular and challenging Cityscapes dataset with video object segmentations. Results on this new CityscapesVideo dataset show that our approach outperforms all the baselines in this challenging setting.

==> intro_old.tex <==
% !TEX root = top.tex

\section{Introduction}

\hide{
\begin{itemize}
	\item Motivate the task of video instance segmentation, why it's important, its applications, its challenges, 
	\item Talk about the labeling task: How labeling is performed: take motivation from how ATG Seattle did it. 
	\item Break the labeling task into two steps: 1) drawing polygons per frame 2) connecting them in the video. 
	\item Say that this is very time consuming task. Drawing precise polygons is hard. Many points
	\item We require the annotator to specify a single point per object
	\item We also introduce a large scale video segmentation dataset for the task of autonomous driving
\end{itemize}
}


Video instance segmentation, \emph{i.e}. the task of detecting and categorizing the pixels of unique countable objects in space and time, is of paramount interest in many computer vision applications such as autonomous driving, medical imagery, augmented reality and video editing to name a few. In the context of autonomous driving, a typical scene could contain many objects of varying shapes and appearances which have to be precisely delineated from the background and their masks tracked throughout the video. However as the scene evolves, an object could undergo various deformation in both shape and appearance or even become occluded or dis-occluded many times. These challenges render video instance segmentation a very difficult task.   

With the tremendous success of deep learning applied to the image instance segmentation task in the past few years \cite{he2017mask, bai2017deep, ren2017end}, many new such methods and extensions are being developed for the video domain \cite{yang2019video, yang2018efficient, hu2017maskrnn, voigtlaender2019mots}.

These  deep learning methods are very data hungry and demand large scale annotation efforts.  In the single image labeling case, an object instance is annotated by drawing a polygon specifying its boundaries. In case of an object being split due to occlusion or holes, multiple polygons are required. These polygons have to be pixel-level precise that render the annotation task very time consuming. In the video domain,  it is not only required that the polygons delineating the boundaries of objects be very precise,  but they should also be consistent temporally between frames. 

A typical large scale video annotation task consists of two stages. First a group of human annotators draw the polygons for all the objects in all the frames of the video. Next, the polygons corresponding to the same object are linked throughout the video by the annotators. These two stages can be performed with some level of parallelism in annotating  different objects and snippets. The labeling platform usually facilitates the annotation process such that there are no conflicts between the different annotators. Also each stage of the annotation undergoes a review process to assure high quality.  

For efficient large scale annotation, ideally an annotator should only provide minimal cues and later perform quality analysis and correction of a semi-automatically segmented video rather than labeling everything from scratch. One could potentially automate certain parts of each stage of the process. For example for the first stage, an annotator could  either draw a bounding box or specify the 4 extreme points \cite{papadopoulos2017extreme} of an object rather than drawing the whole polygon which is much faster. Next, given these coarse boundaries of the object, one could use an off the shelve state of the art segmentation method \cite{chen2017rethinking} to obtain an initial segmentation or leverage the annotator in the loop line of work \cite{maninis2018deep, PolyRNN, acuna2018efficient, ling2019fast, wang2019object} for interactive segmentation. The model then outputs a segmentation mask \cite{maninis2018deep}, a structured polygon \cite{PolyRNN, acuna2018efficient, ling2019fast},  or a distance field \cite{wang2019object} that can be refined and fed back to the model after user correction. For the second stage, the segmentation masks could be linked using a matching algorithm and verified and corrected by human annotators. 

While these methods speed up the annotation task, still specifying extreme points or  bounding boxes require a heavy cognitive load on the annotator \cite{XXX}. For example, in an autonomous driving scene, there could be many small instances far away occluding each other. Drawing and adjusting the bounding boxes or figuring out the extreme points is time consuming for the annotator taking on average from 7 seconds to 35 seconds per object \cite{XXX}. 

In this paper, we investigate whether we can simplify the task of the annotator so that they are only required to specify an object in the video with a single click anywhere inside the object? 

In particular, we propose an annotator in the loop segmentation model for videos where the user is required to specify the objects with only a single click. Given this single click, a masklet (i.e. a set of consecutive masks) are generated for the object in the snippet. In detail, a siamese network with temporal connections is applied to two consecutive frames to obtain spatio-temporal features. Given a set of keypoints in the first frame specified by the user, we extract their corresponding feature vectors from the spatio-tempral feature map and find their correlation with all the pixels in the second frame to obtain a 3D cost volume. This cost volume indicates the matching of each pixel in the second image to the specified instances in the first frame or to the background. Next, the cost volume is passed to a recurrent attentional network that refines the object masks for a number of iterations. Note that in this paper we create a new masklet for the object if it disappears in one of the frames and reappears again. Furthermore, we ask the users to specify new objects that appear with a single click. 

Also in this paper we introduce a new video instance segmentation dataset by extending the Cityscapes Instance segmentation dataset to video. In particular, we obtain high quality segmentation masks for all the 8 categories of cityscapes. 


 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hide{
	
	
	To do this, one could either use Many methods have been proposed that require an annotator to draw some markers \namdar{cite some traditinal work} that aid the segmentation task and then corre   
	
	
	many deep learning methods have been developed that  \namdar{cite polyrnn, extreme points, scriblles} require the annotator to draw an initial bounding box or specify extreme points corresponding to an object. 
	\namdar{Talk about different datasets}
	
	In interactive segmentation line of work, annotators provide bounding boxes, scribbles, or markers as an input to a segmentation system and then further refine the output. For example the more recent \cite{cite extreme points} provide the 4 extreme points as an extra channel to a deep network which outputs a guided segmentation mask. If there is room for improvement, more points on the boundary are provided to the system.  
	
	
	To ease annotation efforts, many methods are 
	
	\section{Skeleton:}
	
	\begin{enumerate}
		\item Define video instance segmentation
		\item Talk about applications
		\item Talk about deep learning methods being applied to this task
		\item Say that these methods are very data hungary. Talk about some datasets.
		\item Annotation is very time consuming.
		\item In this paper, we develop an annotator in the loop method to tackle these challenges.
		
	\end{enumerate}
	
	
	
	
	\section{Notes}
	
	
	\begin{itemize}
		\item Talk about instance segmentation and why it's important.
		
		\item it would be more cost effective for the annotators to perform manual QA or correction of some initial segmentation masks.  For the single image task
		
		\item  In contrast to the  image level instance segmentation task, in video one has to deal with  
		
		Have to reason about all the pixles. 
		
		\item Talk about the importance of instance segmentation in videos and shortcoming
		
		The task of instance segmentation, that is assigning to countable objects in the image such as cars, people, animals , etc each pixel in the image its category  
		
		That is inferring the pixels corresponding to countable objects in the scene such as vehicles, people and animals, 
		
		\paragraph{Applications:}
		Image simulation, action recognition from video, intent prediction from video, augmented reality, image inpaiting
		
		
		\item The importance of instance segmentation in autonomous driving. 
		GT data for simulation models.
		Multiple intersecting bounding boxes are ambiguous but the pixels are more informing.  
		
		\item 
		
		\paragraph{Difficulties} Talk about why temporal coherency is important in videos, 
		
		flickering, inconsistent boundaries.
		
		\item Talk about how we tackle this problem. 
		
		To tackle these challenges, in this paper we formulate the problem of consistent instance segmentation as one of inference in a deep structured model.
		
		In this paper, we formulate the problem as inference in a deep structured model. In particular, a deep network provides features fro the classic and powerful Chan-Vese level set method. 
		
		Wen thoroughly evaluate the effectivness of our model on multiple datasets. 
		
		Annotator in the loop: Given tracked bounding boxes of objects, output a a structured representation of the object in space and time.
		
		How is video annotation done?
		
		\item What's the scope? autonomous driving or other datasets as well?
		
		\item{Annotation:} 
		
		\item Pixel level object segmentation in videos is a very time consuming task. For example, annotating each object such a such as cars with polygons takes on average \XXX seconds per image. For a video of 5 seconds at 10 FPS, this amounts to \XXX which is a lot. On the other hand, annotating bounding boxes/extreme points for the object of interest in the video is much faster at an average of \XXX per instance in each image.   
		
		
		\item Image instance segmentation is the task of identifying the pixels in the image corresponding to countable objects in the scene and predicting their category. With the advent of deep learning in the past decade, this task has seen tremendous success. Video instance segmentation extends this to temporal frames. 
		
		One of the biggest challenges in video instance segmentation is the temporal coherency of the object mask and boundaries. 
		
		
		
	\end{itemize}
	
	
	\section{Experiments}
	
	\section{Ideas}
	
	\begin{itemize}
		\item Say we segment a video of N frames. An annotator comes and looks at a subset M of the frames and either says they're good or fixes them. This signals that  M of them are GT now. How can we leverage these M frames to improve the rest?
		\item active learning
	\end{itemize}
	
	
	\begin{itemize}
		\item Kitti MOTS
		\item Youtube VOS
		\item Youtube VIS
	\end{itemize}
	
}

